Recent Advances in Hate Speech Moderation: Multimodality and the Role of Large Models

In the evolving landscape of online communication, moderating hate speech (HS) presents an intricate challenge, compounded by the multimodal nature of digital content. This comprehensive survey delves into the recent strides in HS moderation, spotlighting the burgeoning role of large language models (LLMs) and large multimodal models (LMMs). Our exploration begins with a thorough analysis of current literature, revealing the nuanced interplay between textual, visual, and auditory elements in propagating HS. We uncover a notable trend towards integrating these modalities, primarily due to the complexity and subtlety with which HS is disseminated. A significant emphasis is placed on the advances facilitated by LLMs and LMMs, which have begun to redefine the boundaries of detection and moderation capabilities. We identify existing gaps in research, particularly in the context of underrepresented languages and cultures, and the need for solutions to handle low-resource settings. The survey concludes with a forward-looking perspective, outlining potential avenues for future research, including the exploration of novel AI methodologies, the ethical governance of AI in moderation, and the development of more nuanced, context-aware systems. This comprehensive overview aims to catalyze further research and foster a collaborative effort towards more sophisticated, responsible, and human-centric approaches to HS moderation in the digital era. WARNING: This paper contains offensive examples.

==> OLD/future_directions.tex <==
To conclude this survey, we explore prospective research opportunities in utilizing large-scale models for moderating hate content.

% \subsection{Hate Speech Generation}
% Previous studies have explored the use of generative networks to generate adversarial examples for hate speech. HateGAN \cite{cao2020hategan} trains a generative adversarial network (GAN) architecture to generate synthesised hateful tweets, which addresses the imbalance of hate speech to non-hate speech. memeBot \cite{} trains a encoder-decoder transformer model to produce a meme, given a meme and a input prompt. More recently, Qu et al. \cite{} explores the use of text-to-image models on generating unsafe images and hateful memes, which highlights the dangerous potential of generating hate speech with artificial intelligence.



% \subsection{Hate Speech Explanation}
% Recent research has demonstrated promising results in prompting large language models to produce meaningful explanations for hate speech. In their study, Wang et al. \shortcite{wang2023evaluating} found that explanations for hate speech generated by GPT-3 are quite persuasive and sound, as evidenced by extensive human evaluations. Additionally, \textsf{HARE} \cite{yang2023hare} introduced two methods for creating rationales for hate speech. These methods were then utilized to enhance the training of a hate speech detection model, resulting in improved performance. 

% \paragraph{Hate Speech Explanation.} Although current methods in HS explanation using large-scale models (refer to Section \ref{sec:hate-speech-explanation}) have shown promise, they still face significant challenges. These large models are prone to ``hallucinations," producing responses that can be factually incorrect, illogical, or unrelated to the initial prompt \cite{ji2023survey}. Consequently, while these recent advancements are promising, the explanations generated by these models are susceptible to misinformation and require verification. Future research should aim to improve the accuracy and relevance of these explanations. This might involve anchoring the explanations in verifiable facts and developing techniques to identify and rectify any discrepancies.

% \paragraph{Cross-Modality Transfer Learning.} Cross-modality transfer learning is a paradigm of learning that allows the transfer of learned knowledge across a modality. In a typical scenario, this approach might be applied when the learned distribution and the test distribution are significantly different. In a hateful textual context, researchers have used a large amount of translated data from English to fine-tune a  multilingual pre-trained BERT or fine-tune a multichannel BERT with parallel translated data. They observed partial success in both of the approaches \cite{casula2020transfer}. In some cases, researchers tried to formulate the task of cross-modality in the form of cross-task learning \cite{yang2022multimodal}. Here, the task of hate detection was considered primary, whereas the task of sarcasm detection was considered as the auxiliary one. Although both tasks have a high correlation, researchers were able to identify a total of three gaps -- a semantic gap that is caused by the inconsistencies of the images and corresponding texts; a domain gap caused by different sources of information, and a definition gap due to the different standardization of the definition. They used the Facebook Hateful Memes dataset and the Twitter Sarcasm dataset. The authors incorporated contrastive learning, weighted sampling, and conditional domain adversarial network \cite{long2018conditional} to reduce the semantic gap, definition gap, and domain gap respectively.

\paragraph{Cross-Modality Context Understanding.} As hate speech extends beyond mere text to encompass multiple forms of media (multimodality), it becomes crucial for models to possess a proficient understanding of context across these different modalities. Hence, it is imperative that models not only identify hateful content within text or images separately but also grasp how the combination of text and images can alter the overall message \cite{DBLP:conf/nips/KielaFMGSRT20}. For instance, an image that is benign on its own might become hateful when paired with specific text. Research could focus on developing models that more effectively understand context across different modalities.

\paragraph{Low-Resource Hate Speech Adaptation.} Domain adaptation between related tasks has gained significant attention, with transfer learning emerging as a prominent strategy for addressing this challenge. In the domain of hate speech, an exemplary application is the cross-lingual transfer learning for detecting hate speech across different languages. Winata et al. \cite{winata2022cross} use few-shot in-context learning and fine-tuning techniques to adapt insights from languages with abundant resources to those with fewer resources. Given the widespread presence of hate speech and its relatively consistent definitions across different forms, there is potential to extend knowledge from text-based hate speech with abundant resources to other low-resource forms of hate speech. Future research should aim to develop models capable of pre-training on a broad spectrum of multimodal data, including text, images, audio, and videos, to enhance transfer learning capabilities.

\paragraph{Humour \& Sarcasm Understanding.} Comprehending humor and sarcasm involves recognizing subtle linguistic signals and understanding the broader context, which includes cultural, social, and environmental factors. LLMs are adept at processing language but might not entirely capture these intricate details or fully understand the specific circumstances surrounding a statement. Additionally, humor and sarcasm often hinge on wordplay, double meanings, or ambiguous interpretations. Although LLMs can identify language patterns, they might struggle to differentiate between straightforward and figurative speech. Research efforts can focus on enhancing the capability of LLMs and LMMs to interpret sarcasm and humor, particularly dark humor, which conceals itself within the context of a sentence.

\paragraph{Multicultural Moderation.} A challenge in hate speech detection lies in the varying cultural and contextual cues across different countries and regions. These subtle cues often require a nuanced understanding of local languages, dialects, slang, and social norms. This complexity makes it difficult for automated systems to identify and differentiate hate speech from non-offensive content. Nguyen et al. \cite{nguyen2023extracting} demonstrated how providing cultural common-sense knowledge can alter GPT-3’s behaviour, leading it to produce more accurate and culturally sensitive questions. Similarly, future research could aim to curate HS dataset with regional culture information and build culturally-aware LLMs and LMMs by injecting and fine-tuning models with cultural knowledge.

\paragraph{Real-Time Monitoring.} The vocabulary of hate speech is constantly changing and evolving, particularly in online spaces. Although adapting to different domains can enhance a model's capacity to apply its knowledge across a range of current datasets, the ongoing development of new slurs, coded terms, and symbolic expressions presents a considerable obstacle to the successful detection of hate speech. Research efforts can focus on continual learning methods that enable these models to be updated regularly while minimising the adjustments to their parameters.

\paragraph{Factual Grounding.} Although current methods in generating HS explanation using large-scale models (refer to Section \ref{sec:hate-speech-explanation}) have shown promise, they still face significant challenges. These large models are prone to ``hallucinations" producing responses that can be factually incorrect, illogical, or unrelated to the initial prompt \cite{ji2023survey}. Consequently, while these recent advancements are promising, the explanations generated by these models are susceptible to misinformation and require verification. Future research should aim to improve the accuracy and relevance of these explanations, which might involve anchoring the explanations in verifiable facts and developing techniques to identify and rectify any discrepancies.

==> OLD/hate_speech.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=1.0\linewidth]{images/survey-taxonomy.pdf}
\caption{Typology of HS based on modalities and tasks. The dark blue boxes are mature research areas with multiple studies; light grey boxes are ongoing research areas, while the hat can be found, and hatched boxes are unexplored topics.}
\label{fig:typology}
\vspace{-3mm}
\end{figure}

HS takes various forms — written text, images, spoken words, and multimedia content — each posing risks of violence, animosity, or prejudice against specific groups. This section reviews existing literature on HS, categorizing it into text-based, image-based, video-based, and audio-based types. Figure \ref{fig:typology} illustrates the range of online HS forms. Additionally, Table 1 lists publicly accessible HS datasets for different modalities, providing researchers with essential resources for data collection and analysis, and supporting comprehensive and consistent research in HS detection and moderation.

%Hate Speech, manifesting in diverse forms such as written text, images, spoken words, and even multimedia content, poses significant risks, leading to violence, animosity, or prejudice against specific groups. This section delves into the extant literature on HS, emphasizing its unique challenges and categorizing its various forms into four distinct types: \textit{text-based HS}, \textit{image-based HS}, \textit{video-based HS}, and \textit{audio-based HS}. Figure \ref{fig:typology} presents an overview typology, encapsulating the wide spectrum of online HS forms.

%Table 1 provides a detailed compilation of publicly accessible datasets for HS across different modalities. These datasets serve as valuable resources, streamlining the data gathering and selection process for researchers. They offer a foundational platform for conducting thorough and consistent analyses in diverse research projects within the field of HS detection and moderation.

%Hate speech manifests in various forms, including written words, images, and spoken words, and can lead to violence, animosity, or prejudice against specific groups. This section explores the current literature on hate speech, focusing on its distinct challenges and various tasks in three different forms: \textit{text-based hate speech}, \textit{image-based hate speech}, \textit{video-based hate speech} and \textit{audio-based hate speech}. Figure \ref{fig:typology} illustrate the overview typology that covers the diverse forms of online hate speech.

\subsection{Text-based Hate Speech}
Text-based HS encompasses written or typed expressions manifesting across various digital formats, including social media posts \cite{waseem2016hateful,founta2018large}. Researchers addressing online HS have compiled datasets to detect and analyze its complexity and multifaceted nature, as detailed in existing literature. These studies explore diverse aspects of hateful and derogatory language, focusing on themes such as implicit HS \cite{elsherief2021latent}, targeted groups \cite{kennedy2018gab}, and types of attacks \cite{elsherief2021latent}. As detection models evolve, it becomes imperative to understand and elucidate their decision-making processes, leading to the development of datasets for implicit statements and methodologies for bias analysis \cite{sap2019social,elsherief2021latent}. Additionally, some research shifted towards proactive strategies, including countering HS \cite{masud2022proactively}.

%Text-based hate speech refers to written or typed expressions that occur in various formats, including social media posts \cite{waseem2016hateful,founta2018large,fersini2018overview}, online comments \cite{rieger2021assessing,hiaeshutter2022language}, forums \cite{doring2020gendered,obadimu2019identifying}, and other digital platforms. 
%To address the issue of online hate speech, researchers have collected datasets to detect text-based hate speech on the internet, examining its complex and multifaceted nature as discussed in existing literature. These studies investigate various aspects of hateful and derogatory language, such as implicit hate speech \cite{vidgen2021learning,hartvigsen2022toxigen}, attacked target(s) \cite{kennedy2018gab,basile2019semeval}, attacked type(s)\cite{elsherief2021latent}. As detection models improve, understanding and explaining their decision-making processes become crucial, leading to the creation of datasets for implied statements \cite{mathew2021hatexplain,sap2019social,elsherief2021latent} and methods for bias analysis. Furthermore, moving past reactive measures, some studies are focusing on proactive strategies like countering and normalizing hate speech \cite{masud2022proactively}.

The detection of text-based HS is fraught with significant challenges. A primary obstacle is contextual understanding; HS often subtly or covertly conveys its message through sarcasm, irony, or cultural references. Linguistic variations, including slang, dialects, and unconventional language forms, exacerbate this intricacy, posing difficulties for automated recognition systems. Additionally, the multilingual nature of online content necessitates language-specific tools or models for effective detection across diverse linguistic contexts. A further complication is the rapid evolution of online language, which can quickly render existing detection models outdated.

%The detection of text-based hate speech presents several significant challenges. The first challenge involves understanding the context, as hate speech often conveys its message subtly or covertly through sarcasm, irony, or cultural references. This complexity is further compounded by language variations such as slang, dialects, and unconventional forms of language, which can hinder automated recognition systems. Moreover, the presence of content in multiple languages requires a range of language-specific tools or models for effective detection across different linguistic contexts. An additional obstacle is the rapid evolution of language, particularly online, which can quickly render current detection models obsolete.

% Current literature \cite{elsherief2021latent,sap2019social} categorizes hate speech into two distinct forms: \textit{explicit} and \textit{implicit} hate speech. 

% Explicit hate speech is direct and unambiguous, clearly expressing derogatory views or inciting harm against a specific group. It often involves the use of slurs, derogatory language, and outright threatening or demeaning statements. In contrast, implicit hate speech is more subtle and often disguised, conveying discriminatory sentiments through coded language or stereotypes. This form of hate speech can be particularly harmful because it subtly reinforces prejudice and discrimination, shaping attitudes and actions without explicitly displaying bigotry. We observe that these distinctions continue to exist across different modalities, with implicit hate speech becoming more prevalent
% Furthermore, lexicon-based approaches face challenges in keeping pace with the dynamic evolution of language, especially on online platforms where new jargon and phrases continuously emerge. 
% RNNs and Transformers can be trained on large datasets to learn patterns and nuances in language, making them more adaptable to different domains or styles of text. 

% \textbf{Methodologies \& Challenges}. Current research focuses on developing methodologies either based on lexicons or at the sentence level. Popular lexicon-based methods involve constructing a lexicon corpus \cite{gitari2015lexicon} or training a supervised classifier using an N-gram \cite{oriola2020evaluating}. These techniques are particularly advantageous for addressing hate speech in languages with limited resources, where data availability is a significant constraint. However, these methods tend to overlook the broader sentence context and subtle linguistic variations. They often rely excessively on specific words or phrases, leading to potential misinterpretations of expressions that are nuanced or highly context-dependent. Sentence-level approaches alleviate these limitations by using deep neural networks, such as RNN and Transformer architecture, to capture context and understand the meaning of words in relation to their surrounding words. Nevertheless, these techniques are still susceptible to lexicon-level bias, which remains an area for future research exploration to develop a more generalizable system.

\subsection{Image-based Hate Speech}
% Image-based hate speech employs visuals, such as photographs, cartoons, and illustrations, to promote hate or discrimination against specific groups. A prevalent form of this hate speech is memes, which typically comprising images with short overlaid texts. While memes are often humorous or satirical, they are increasingly being exploited to disseminate hateful content online. Furthermore, the viral nature of memes on digital platforms make this type of hate speech particularly influential, as it can spread rapidly and reach a wide audience. Recent studies have focused on the substantial influence and prevalence of image-based hate speech, especially in memes. Researchers have developed datasets for detecting hateful memes \cite{DBLP:conf/nips/KielaFMGSRT20,DBLP:conf/wacv/GomezGGK20,DBLP:conf/case-ws/ThapaSJNR22} and are exploring various aspects of this issue. Some studies are investigating the identification of specific targets within these memes \cite{mathias-etal-2021-findings,DBLP:conf/semeval/FersiniGRSCRLS22}, while other studies are examining the understanding \cite{DBLP:conf/www/HeeLC22,DBLP:journals/ipm/RizziGSRF23} \crcomment{Here, would it be better if we explicitly point they study bias? First is to align with teh typology figure. Secondly,~\cite{DBLP:journals/ipm/RizziGSRF23} considered beyond analyzing bias but also mitigation of bias.} and explanation \cite{DBLP:conf/ijcai/HeeCL23,DBLP:conf/emnlp/LinLMC23} of the methods behind visual hate speech. Additionally, recent explorations are being conducted into strategies for countering hate speech in memes \cite{DBLP:journals/corr/abs-2311-06737}.~\crcomment{Would we update the typology figure? Explanation, counter hate speech have been explored for image-based hate speech. To distinguish from audio and video based ones, shall we change the color of the blocks (e.g., change color of explanation and counter speech block to be the same as the bias one)}

Image-based HS utilizes visual elements, such as photographs, cartoons, and illustrations, to propagate hate or discrimination against specific groups. A common manifestation of this type is memes, which typically consist of images combined with short overlaid text. Although memes often serve humorous or satirical purposes, they are increasingly used to spread hateful content online \cite{DBLP:conf/nips/KielaFMGSRT20}. The viral nature of memes on digital platforms further amplifies their impact, allowing them to reach vast audiences rapidly. To address the proliferation of hateful memes, recent studies have focused on developing datasets for their detection \cite{DBLP:conf/nips/KielaFMGSRT20,DBLP:conf/wacv/GomezGGK20} and for identifying specific targets and types of attacks within these memes \cite{DBLP:conf/semeval/FersiniGRSCRLS22}. Beyond detection, new approaches are being pursued to analyze and mitigate bias in image-based HS detection models \cite{DBLP:conf/ijcai/HeeCL23,DBLP:conf/emnlp/LinLMC23}. Additionally, new methodologies are emerging to counteract HS transmitted through memes \cite{DBLP:journals/corr/abs-2311-06737}.

%Image-based hate speech employs visuals, such as photographs, cartoons, and illustrations, to promote hate or discrimination against specific groups. A prevalent form of this hate speech is memes, which typically comprise images with short overlaid texts. While memes are often humorous or satirical, they are increasingly being exploited to disseminate hateful content online. Furthermore, the viral nature of memes on digital platforms makes this type of hate speech particularly influential, as it can spread rapidly and reach a wide audience. To curb the dissemination of hateful memes, recent studies have developed datasets for detecting hateful memes \cite{DBLP:conf/nips/KielaFMGSRT20,DBLP:conf/wacv/GomezGGK20,DBLP:conf/case-ws/ThapaSJNR22} and the identification of specific targets and attack types within these memes \cite{mathias-etal-2021-findings,DBLP:conf/semeval/FersiniGRSCRLS22}. Aside from detection, new methods are being devised to analyze and reduce bias in image-based hate speech detection models \cite{DBLP:conf/ijcai/HeeCL23,DBLP:conf/emnlp/LinLMC23}. Furthermore, new strategies are being explored to counteract hate speech conveyed through memes \cite{DBLP:journals/corr/abs-2311-06737}.

Detecting image-based HS presents challenges due to the nuanced expression of offensive messages in visual content. Images, often embedding symbols, memes, or culturally specific visual cues, require deep cultural and contextual understanding for accurate interpretation. The combination of visual elements and text can subtly imply meanings not immediately evident \cite{DBLP:conf/nips/KielaFMGSRT20}. For example, Figure 1 depicts a man with a gun and text suggesting hostility towards immigrants. Differentiating humor from hate in memes is particularly challenging, influenced by varying cultural, societal, and personal perspectives \cite{schmid2023humorous}.

%The detection of image-based HS poses unique challenges due to the nuanced and complex ways visual content can express offensive messages. Images often incorporate symbols, memes, or visual cues with cultural specificity, requiring a deep understanding of both culture and context for accurate interpretation. Additionally, the integrated analysis of visual elements and overlaid text often reveals subtly implicit meanings that might not be immediately apparent \cite{DBLP:conf/nips/KielaFMGSRT20}. For instance, Figure 1 shows an image of a man aiming a gun, accompanied by the text ``\textit{see an illegal immigrant mowing their lawn}" covertly expressing animosity towards immigrants. A particularly complex aspect is distinguishing between humor and hate in memes, which can vary significantly based on cultural, societal, and individual perspectives \cite{schmid2023humorous}.

%The detection of image-based hate speech presents unique challenges due to the nuanced and varied ways in which visual content can convey offensive messages. Images may incorporate symbols, memes, or visual cues that are culturally specific, conveying hate speech in a manner that demands both cultural knowledge and contextual understanding for accurate interpretation. Moreover, the simultaneous analysis of visual elements and overlaid text in an image can reveal subtly implicit meanings that were not apparent before \cite{DBLP:conf/nips/KielaFMGSRT20}. For example, Figure 1 depicts a man aiming a shot, coupled with the text ‘’see an illegal immigrant mowing their lawn’’, implicitly communicating animosity towards illegal immigrants. Most importantly, there is increased ambiguity between humorous and hateful memes, which often depend on cultural, societal, and individual perspectives \cite{schmid2023humorous}. 

\subsection{Video-based Hate Speech}
Video-based HS presents a complex challenge, comprising a blend of visuals, audio tracks, and/or textual elements. This form of HS ranges from professionally produced propaganda to amateur videos on social media platforms like YouTube and TikTok. The engaging nature of video content and its easy dissemination across digital networks significantly heighten its potential for harm. Echoing the concerns of image-based HS, video-based HS also contributes to the normalization of hateful ideologies and can profoundly influence public opinion. Contemporary research in this domain primarily focuses on identifying video-based HS and categorizing its various subtypes \cite{wu2020detection}. Recent studies have explored detecting hateful segments within videos alongside multi-dimensional analysis. Nonetheless, the body of research on video-based HS is less developed than text-based and image-based HS, particularly in areas such as analyzing and mitigating model bias, elucidating decision-making processes, and devising counterstrategies. These gaps, likely stemming from the rapid pace of technological advancements and evolving digital trends, underscore the need for further research to promote a more harmonious online environment.

%Video-based hate speech represents a particularly challenging problem, involving a series of visuals enhanced by elements like an audio track and/or text. This type of hate speech varies widely, from professionally crafted propaganda to amateur videos posted on social platforms like YouTube and TikTok. The engaging nature of video content, coupled with the ease of distribution across digital networks, amplifies its potential for harm. Similar to image-based hate speech, video-based hate speech can normalize hateful ideologies and significantly impact public opinion. Current research in this area focuses on identifying video-based hate speech \cite{de2020self,ibanez2021audio} and classifying various subtypes of hate \cite{wu2020detection}. A recent study delved into detecting hateful segments within video-based hate speech, along with conducting multi-dimensional analysis. However, compared to the literature for text-based and image-based hate speech, there is a noticeable gap in the video-based hate speech literature, particularly regarding the analysis and mitigation of model bias, explanation of the decision-making process, and the development of countermeasures. These gaps, likely due to recent technological advancements and digital trends, present opportunities for future research aimed at fostering a more harmonious society.

Identifying HS within videos is a demanding and resource-intensive endeavor. This complexity stems from the amalgamation of various elements, such as text, images, and audio, within a single medium. Each component can independently harbor HS, thereby compounding the detection process. The duration of videos further exacerbates this challenge, as longer content necessitates more extensive review and analysis, with potential shifts in context over time. Moreover, subtle visual cues and sophisticated editing techniques can be employed to discreetly embed hate messages, making their detection by automated tools particularly challenging. Additionally, the analysis of video content requires considerable computational resources and time, posing a substantial challenge for organizations tasked with detecting and addressing HS in video formats.
%\todo{the entire last paragraph is uninformative and vague}

%Identifying hate speech in videos is a challenging and resource-demanding task. This complexity arises from the integration of different elements like text, images, and audio into a single format. Each element can independently contain hate speech, making the detection process more complex. The length of videos adds to the difficulty as longer content takes more time to review and analyze, with the possibility of changing contexts throughout the video. Subtle visual signals and editing methods can also be used to convey hate messages subtly, which are hard to detect with automatic tools. Moreover, analyzing videos requires substantial computational power and time, presenting a significant challenge for entities trying to detect and address hate speech in video content.

\subsection{Audio-based Hate Speech}
Audio-based HS entails the analysis of sound waves to discern elements such as pitch, intonation, and the contextual meaning of spoken words. This form of HS can originate from a variety of audio channels, including real-time conversations, podcasts, broadcasts, and other forms of audio media. The methodologies for addressing audio-based HS are diverse, targeting different facets of the issue. For instance, Barakat {\em et al.} \shortcite{6376654} employed a straightforward keyword-based approach to identify segments of HS, while Wazir {\em et al.} \shortcite{9287133} engaged in a detailed classification of offensive categories in audio-based HS, showcasing a nuanced method of understanding and categorizing this form of HS. This research area is still in its developmental stages, partly due to the scarcity of dataset. Nonetheless, recognizing the variety and significance of the approaches and techniques employed in this field is imperative. This recognition not only sheds light on the current state of research but also illuminates potential avenues for future exploration.

%Audio-based hate speech primarily involves analyzing sound waves to understand elements such as pitch, intonation, and the context of spoken words. This type of hate speech can be sourced from various audio channels, including real-time conversations, podcasts, broadcasts, and other audio media. The approaches to tackle audio-based hate speech are diverse, addressing different aspects of the issue. For example, one study \cite{6376654} adopted a simple keyword-based method to identify hateful speech segments. On the other hand, another research \cite{9287133} delved into a fine-grained classification of foul categories in audio-based hate speech, illustrating a distinct way of understanding and categorizing hate speech. The body of research in this area is still evolving, partly due to the limited availability of audio samples containing hate speech. However, it's crucial to acknowledge the variety and importance of the tasks and techniques used in this field, which also highlight potential areas for future research.

Detecting HS in audio recordings presents unique challenges, primarily related to the transcription and interpretation of spoken words. The accuracy of speech recognition is crucial, especially when dealing with diverse accents, background noise, or poor audio quality. Additionally, the tone and intonation of spoken language play a significant role in conveying intent, which can substantially alter the meaning of words. This aspect poses a challenge for detection based solely on text transcripts, as subtle nuances in vocal expression may be lost during transcription. Moreover, non-verbal audio elements, such as sound cues or background noises, are pivotal in contextualizing speech. However, these elements are often difficult to interpret using automated methods.

%Detecting hate speech in audio recordings poses distinct challenges, primarily arising from transcribing and comprehending spoken words. The accuracy of speech recognition emerges as a critical factor when confronted with diverse accents, ambient noise, or subpar audio quality. Furthermore, the tone and intonation of spoken language wield considerable influence in conveying intent, often altering the perception of individual words. This makes it challenging to detect hate speech based solely on text transcripts, as nuances in vocal expression are often lost in translation. Additionally, non-verbal sounds, such as audio cues or background noises, can be significant in understanding the context of speech, but these are hard to interpret through automated means.

% The methods employed in these studies are diverse and tailored to the specific challenges of each task. For detecting offensive words in spontaneous, user-generated content, time series analysis techniques and speaker-independent feature extraction methods were effectively used in \cite{6376654}. In contrast, \cite{SoniEvil} integrated a multimodal analysis approach, combining audio, visual, and textual data, to enhance the effectiveness of cyberbullying detection. Furthermore, the study \cite{9287133} utilized machine learning models like neural network-based architectures for fine-grained foul category classification. Additionally, the study \cite{s21030710} focused on foul language identification using various neural network approaches including feedforward, recurrent, and memory-enhanced neural networks, demonstrating the efficacy of feedforward neural networks in a two-class problem with high F1 scores.

%\subsection{Hate Speech Datasets}

%Table 1 shows a comprehensive listing of publicly accessible datasets for hate speech in various modalities. These comprehensive resources are intended to simplify the process of gathering and choosing data, establishing a solid basis for thorough and consistent analysis in various research endeavors within this field.


==> OLD/method.tex <==
In this section, we review state-of-the-art methodologies that have made significant contributions to key areas of HS research: \textit{HS detection}, \textit{HS explanation}, \textit{HS debiasing}, and \textit{counter speech}. We emphasise research studies incorporating LLMs or LMMs, aiming to garner comprehensive insights into emerging trends within this domain. This allows us to understand how these advanced models enhance our understanding and management of HS in various forms.

%In this section, we have chosen and reviewed several state-of-the-art methodologies that have significantly contributed to distinct areas of hate speech research: \textit{hate speech detection}, \textit{hate speech explanation}, \textit{hate speech debiasing} and \textit{counter speech}. Our focus is on research studies that incorporates large multimodal models to obtain a more comprehensive insights into the emerging trend in this research domain.

\subsection{Large Models}
% The emergence of large foundation models, such as LLMs and LMMs, has revolutionized the research landscape by exhibiting impressive generative capabilities along with new emergent abilities \cite{zhao2023survey}. LLMs excel at tasks involving text comprehension and generation \cite{touvron2023llama}. In contrast, LMMs are adept at processing various data types, including visual, textual, and auditory inputs, which enables a broad spectrum of applications. In this survey, we regard both LLMs and LMMs as models with several billion parameters, aligning with the definition widely accepted and analyzed in numerous studies of large-scale models \cite{luo2023zero}.

The emergence of large foundation models, such as LLMs and LMMs, marks a significant milestone in artificial intelligence research, showcasing unprecedented capabilities in understanding and generating data across different formats  \cite{zhao2023survey}. LLMs are designed to excel in language understanding and text generation  \cite{touvron2023llama}. In contrast, LMMs are adept at processing and interpreting various data types, including visual, textual, and auditory inputs, enabling a broader spectrum of applications \cite{yang2023dawn}. These foundation models have opened new avenues for identifying and mitigating hateful content, which requires nuanced understanding of language and context.

In this survey, we regard both LLMs and LMMs as models with several billion parameters, aligning with the definition widely accepted and analyzed in numerous studies of large-scale models \cite{luo2023zero}.

% - Multimodal: yawn2023dawn - The Dawn of LMMs


\subsection{Hate Speech Detection}
% The existing detection techniques varies across the various forms of hate speech, encompassing a range from transformer-based models to spectrogram-based classification models. DeepHate \cite{awal}

% The existing state-of-the-art detection techniques varies across the various forms of hate speech, encompassing a range from transformer-based models to spectrogram-based classification models. AngryBERT \cite{awal2021angrybert} adopts a multi-task learning approach to fine-tune BERT on suitable co-training tasks for binary text-based hate speech detection. PromptHate \cite{DBLP:conf/emnlp/CaoLC022} adopts a combination of in-context learning and demonstration sampling strategy to perform mask prompt fine-tuning on RoBERTa model for hateful memes detection. \textcolor{red}{mention for video and audio}. 

The leading detection techniques for HS vary according to the modality of the content, encompassing approaches from transformer-based models to spectrogram-based classification models. For instance, AngryBERT \cite{awal2021angrybert} employs a multi-task learning approach to fine-tune  BERT specifically for binary text-based HS detection. 
% It achieves F1-scores of 0.8125, 0.9071, and 0.8108 on the WZ-LS, DT, and FOUNTA datasets, respectively. 
PromptHate \cite{DBLP:conf/emnlp/CaoLC022} integrates in-context learning with a demonstration sampling strategy for mask prompt fine-tuning on RoBERTa, targeting hateful memes. 
% This method attained an AUC score of 0.8145 on the FHM dataset. 
In audio-based HS classification, studies \cite{boishakhi2021multi,ibanez2021audio} have leveraged ensemble techniques involving AdaBoost, Naive Bayes, and random forest.
% , achieving accuracies of up to 0.87 and 0.785. 
Additionally, CNNs have been utilized to convert audio into spectrograms \cite{Medina2022}, with self-attentive CNNs \cite{9616001} employed to extract audio features. For video-based HS classification, a combination of BERT, ViT, and MFCC has been used for text, image, and audio modality analysis, respectively \cite{das2023hatemm}.
% , yielding an accuracy of 0.798 and an F1 score of 0.748 on a specific dataset \cite{das2023hatemm}. 
Note that video-based and audio-based HS detection represent emerging fields, offering substantial scope for further development and innovation.

%The current top-performing detection techniques for hate speech vary depending on the form of hate speech, ranging from transformer-based models to spectrogram-based classification models. AngryBERT \cite{awal2021angrybert} utilizes a multi-task learning approach to fine-tune the BERT model on specific co-training tasks for binary text-based hate speech detection, achieving F1-scores of 0.8125, 0.9071, and 0.8108 on the WZ-LS, DT, and FOUNTA datasets, respectively. PromptHate \cite{DBLP:conf/emnlp/CaoLC022} combines in-context learning with a demonstration sampling strategy to perform mask prompt fine-tuning on the RoBERTa model for detecting hateful memes, achieving an AUC score of 0.8145 on the FHM dataset. In the direction of audio-based hate speech classification, \cite{boishakhi2021multi,9675250} heavily relied on ensemble techniques based on AdaBoost and Naive Bayes and random forest, securing up to 0.87 and 0.785 accuracy, respectively. Others have used CNN to convert audio into spectrograms \cite{Medina2022}, self-attentive CNNs \cite{9616001,s21030710} to extract audio features. For video-based classification, the authors have achieved an accuracy of 0.798 and an F1 score of 0.748 on their prescribed dataset using the combination of BERT, ViT, and MFCC together to utilize classification features for text, image, and audio modality, respectively \cite{das2023hatemm}. Additionally, it is important to note that video-based and audio-based hate speech detection are still emerging areas of research, presenting opportunities for further advancement and improvement.

% While text-based hate speech detection have achieved impressive performance using transformer-based models, a main challenge lies in generalizing to out-of-distribution datasets. This limitation can be attributed to their limited vocabulary and the scarcity of implicit hate speech in many datasets \cite{ocampo2023depth}. Recent approaches addressing this issue with large language models include the generation of adversarial hate speech \cite{cao2020hategan,ocampo2023playing} and in-context learning \cite{wang2023large}. Ocampo \shortcite{ocampo2023playing} introduced a framework that utilizes GPT-3 to create implicit hate speech, thereby confusing and subsequently enhancing hate speech classifiers. Meanwhile, Wang \shortcite{wang2023large} designed a technique for selecting and employing optimal examples in in-context learning for large language models. Whereas, image-based hate speech detection mainly struggles with the complexity of interpreting the implicit hate message. This challenge often arises due to information loss during the extraction of text-based visual features from memes, a common process in many approaches \cite{DBLP:conf/mm/LeeCFJC21,pramanick2021momenta,DBLP:conf/emnlp/CaoLC022}. Additionally, implicit hate speech in memes can be disguised by the seemingly unrelated text and images, as shown in Figure 1. To mitigate the information loss in the image-to-text conversion, ProCap \shortcite{DBLP:conf/mm/CaoHKCL023} prompts a vision-language model in a question-answering format, which improves the quality and informativeness of the generated caption. On the other hand, to address the issue of seemingly unrelated text and image, MR.HARM \shortcite{DBLP:conf/emnlp/LinLMC23} prompts a large language model to generate potential rationales. These rationales are then used to fine-tune supervised hate speech classification systems through knowledge distillation, thereby enhancing the detection of hateful memes.

Transformer-based models have significantly advanced the detection of text-based and image-based HS; yet they encounter specific challenges. For text-based models, a major hurdle is generalizing to out-of-distribution datasets, often hindered by limited vocabulary and the rarity of implicit HS in many datasets \cite{ocampo2023depth}. To overcome this, recent initiatives include adversarial HS generation and in-context learning with LLMs. Ocampo et al. \shortcite{ocampo2023playing} introduced a method using GPT-3 to generate implicit HS, aiming to both challenge and improve HS classifiers. Concurrently, Wang et al. \shortcite{wang2023large} developed a technique for optimizing example selection for in-context learning in LLMs.

In image-based HS, the primary challenge lies in deciphering implicit hate messages within memes. This difficulty often stems from the loss of information during the extraction of text-based features from images, a common step in many methodologies \cite{DBLP:conf/mm/LeeCFJC21,pramanick2021momenta,DBLP:conf/emnlp/CaoLC022}. Furthermore, the implicit HS in memes can be concealed by seemingly unrelated text and images, as illustrated in Figure \ref{fig:hate-speech-modalities}. To address these challenges, recent strategies include employing LMMs with prompting techniques and/or knowledge distillation. ProCap \shortcite{DBLP:conf/mm/CaoHKCL023} addresses the issue of information loss in image-to-text conversion by prompting an LMM in a QA format, enhancing the generated caption's quality and informativeness. To tackle the problem of disconnected text and images, MR.HARM \shortcite{DBLP:conf/emnlp/LinLMC23} utilizes an LMM to generate potential rationales. These rationales are subsequently employed to fine-tune supervised HS classification systems through knowledge distillation, improving the detection of hateful memes.

%Transformer-based models have advanced text-based and image-based hate speech detection, yet they face distinct challenges. there are some challenges impeding their progress. Text-based models struggle with generalization to out-of-distribution datasets, often due to limited vocabulary and the scarcity of implicit hate speech in many datasets \cite{ocampo2023depth}. To address this, recent efforts involve adversarial hate speech generation and in-context learning with large language models. Ocamp \shortcite{ocampo2023playing} introduced a framework utilizing GPT-3 to create implicit hate speech for confusing and subsequently enhancing hate speech classifiers. Meanwhile, Wang \shortcite{wang2023large} designed a technique for selecting and employing optimal examples for in-context learning in larger language models. Conversely, image-based hate speech detection mainly struggles with the difficulty of interpreting the implicit hate message in memes. This challenge often arises due to information loss during the extraction of text-based visual features from memes, which is a common process in many approaches \cite{DBLP:conf/mm/LeeCFJC21,pramanick2021momenta,DBLP:conf/emnlp/CaoLC022}. Additionally, implicit hate speech in memes can be disguised by the seemingly unrelated text and images, as shown in Figure 1. To address these issues, recent efforts involve prompting large models and/or knowledge distillation. To mitigate the information loss in the image-to-text conversion, ProCap \shortcite{DBLP:conf/mm/CaoHKCL023} prompts a large vision-language model in a question-answering format, which improves the quality and informativeness of the generated caption. On the other hand, to address the issue of seemingly unrelated text and image, MR.HARM \shortcite{DBLP:conf/emnlp/LinLMC23} prompts a large language model to generate potential rationales. These rationales are then used to fine-tune supervised hate speech classification systems through knowledge distillation, thereby enhancing the detection of hateful memes.

\subsection{Hate Speech Explanation}
\label{sec:hate-speech-explanation}
A major challenge in contemporary HS detection methods is their lack of explainability in decision-making processes. Explainability is crucial for fostering user trust and facilitating systems that require human interaction \cite{balkir2022necessity}. One proposed solution involves training supervised models that not only categorize HS but also provide rationales for these classifications \cite{sap2019social,elsherief2021latent,DBLP:conf/ijcai/HeeCL23}. Sap {\em et al.} \shortcite{sap2019social} and Elsherief {\em et al.} \shortcite{elsherief2021latent}  developed text-based HS datasets with human-annotated explanations, setting benchmarks for identifying underlying hate. Similarly, Hee {\em et al.} \shortcite{DBLP:conf/ijcai/HeeCL23}  compiled a dataset for hateful memes, complete with human-annotated explanations and benchmarks. However, the process of gathering human-written explanations is not only time-consuming but also susceptible to individual biases. Moreover, it involves the risk of subjecting human annotators to prolonged exposure to HS, which can have adverse psychological effects.
%Existing methods for addressing hate speech often lack explainability in their decision-making processes, which is essential for building user trust and supporting systems that involve human participation \cite{balkir2022necessity}. A suggested approach is to train supervised models that provide not only the classification outcomes but also explanations for these classifications \cite{sap2019social,elsherief2021latent,DBLP:conf/ijcai/HeeCL23}. Both Sap et al. \shortcite{sap2019social} and Elsherief et al. \shortcite{elsherief2021latent} have gathered human-annotated explanations and set benchmarks for underlying hate in their text-based datasets on hate speech. Whereas, Hee et al. \shortcite{DBLP:conf/ijcai/HeeCL23} collected human-annotated explanations and benchmarks for hateful memes. However, collecting human-written explanations is time-consuming and subject to individual biases. Additionally, it poses the risk of exposing human annotators to prolong exposure to hate speech.

Recent studies have delved into employing LLMs to generate plausible and meaningful explanations for HS. For instance, Wang {\em et al.} \shortcite{DBLP:conf/ijcai/WangHACL23} demonstrated that GPT-3 can craft convincing and effective explanations for HS, a finding substantiated by extensive human evaluations. Additionally, {HARE} \cite{yang2023hare} introduces two innovative methods for generating rationales in HS detection, which have been shown to improve both the training process and the performance of detection models. This approach presents an alternative means of developing insightful explanations, while simultaneously mitigating the risks associated with prolonged human exposure to HS. Nevertheless, this area of research is still nascent, thus presenting numerous opportunities for further investigation and development.

%Recent studies have explored the use of large models for generating plausible and meaningful explanations. For instance, Wang et. al \shortcite{DBLP:conf/ijcai/WangHACL23} has shown that GPT-3 can create convincing and effective explanations for hate speech, as confirmed by extensive human evaluations. \textsf{HARE} \cite{yang2023hare} introduces two methods for generating rationales for hate speech, which have been shown to enhance the training and performance of hate speech detection models. This strategy offers an alternative way to develop valuable explanations, while also reducing the prolonged exposure to hate speech. However, this field of research is still emerging, with numerous unresolved issues, opening doors for further exploration and studies.

\subsection{Hate Speech Debiasing}
% Compared with text-based hate speech, there is limited works considering the bias in image-based hate speech detection models. Hee et al.~\cite{DBLP:conf/ijcai/HeeCL23} serves as the very first to quantitatively evaluate the modality bias in image-based hate speech detection models. They found that the image modality contributes more to model predictions. Meanwhile, they highlighted models' sensitivity to certain group identifier terms leads to false-positive predictions. Rizzi et al.~\cite{DBLP:journals/ipm/RizziGSRF23} further analyzed model bias towards detection of misogynous memes. They revealed that  models are biased to terms about stereotypical ideas of women (e.g., \textit{dishwasher} and \textit{broom}). Confronted with the bias, they proposed a mitigation strategy based on Bayesian Optimization, which reduced the bias while maintaining the overall performance.

Bias in HS detection models poses a significant risk to their effectiveness and fairness, leading to potential adverse impacts on individuals and society. Addressing this, numerous studies have focused on identifying and mitigating bias in these models. Sap {\em et al.} \shortcite{sap2019risk} found that two widely-used corpora exhibit bias against African American English, which increases the likelihood of classifying tweets in this dialect as hateful. 
% Further investigations have revealed substantial racial bias across multiple datasets, prompting concerns about racial discrimination in the practical application of these models \cite{davidson2019racial}. 
Hee {\em et al.} \shortcite{DBLP:conf/www/HeeLC22} conducted a quantitative analysis of modality bias in hateful meme detection, observing that the image modality significantly influences model predictions. Their study also highlighted the tendency of these models to generate false positives when encountering specific group identifier terms.

%The risk of bias in hate speech detection models significantly undermines their effectiveness and fairness, causing adverse effects on individuals and society. This has motivated numerous studies to identify bias within these models. Sap et al. \shortcite{sap2019risk} identifies that two widely-used corpus exhibit bias against African American English, leading to a higher likelihood of classifying African American English tweets as hateful. Further research has also uncovered substantial racial bias in multiple datasets, raising concerns about the potential for racial discrimination in practical applications of these models \cite{davidson2019racial}. Hee et al. \shortcite{DBLP:conf/ijcai/HeeCL23} conducted a quantitative analysis of modality bias in image-based hate speech detection models, discovering that image modality heavily influences model predictions. They also noted that models are prone to false positives due to sensitivity to specific group identifier terms. 

Beyond merely identifying biases, various studies have introduced innovative methods to reduce these biases within models. Kennedy \shortcite{kennedy2020contextualizing} developed a regularization technique utilizing SOC post-hoc explanations to address group identifier bias. Similarly, Rizzi {\em et al.} \shortcite{DBLP:journals/ipm/RizziGSRF23} observed that models exhibit biases towards terms linked with stereotypical notions about women, such as \textit{dishwasher} and \textit{broom}. To counteract this, the authors proposed a bias mitigation strategy using Bayesian Optimization, which effectively lessened the bias while preserving overall model performance.

These efforts underscore the critical importance of not only recognizing but actively mitigating bias in HS detection models. This is especially vital as large models increasingly dominate the landscape for generating explanations and enabling transfer learning. Addressing biases within these large models represents a significant opportunity to advance new methodologies and strategies for both the identification and reduction of bias.

%Beyond identifying biases, several studies have proposed novel approaches to mitigate these biases within models. Kennedy \shortcite{kennedy2020contextualizing} proposed a regularization technique that uses SOC post-hoc explanations to mitigate group identifier bias.  Rizzi et al. \shortcite{DBLP:journals/ipm/RizziGSRF23} found that models are biased towards terms associated with stereotypical ideas about women (e.g., \textit{dishwasher} and \textit{broom}) and proposed a mitigation strategy based on Bayesian Optimization, which effectively reduced the bias while maintaining the overall performance.

%$These studies highlight the importance of understanding and mitigating bias in these models, ensuring they neither perpetuate nor amplify biases. As large models become more prevalent for generating explanations and facilitating transfer learning, tackling biases within these large models presents an opportunity to pioneer new approaches and strategies for bias identification and mitigation.

\subsection{Counter Speech}
The approach to counter HS emphasizes creating non-aggressive reactions, aimed at curbing the spread of HS and potentially converting it into respectful and inoffensive language. The primary approach for counter HS involves producing counter-narratives (CN), which rely on reliable evidence, logical arguments, and different perspectives to challenge the hate directed at marginalized groups \cite{chung2021towards}. Multitarget CONAN \cite{fanton2021human} uses GPT-2 to generate potential CN candidates and then engages human evaluators to identify effective CNs, leading to a dataset of $4,078$ CNs. An alternative approach involves either diminishing (i.e., normalization) or eliminating (i.e., correction) the level of hate in HS. NACL \cite{masud2022proactively} employs neural networks to paraphrase sections of text containing hate, effectively lessening the intensity of hate in HS. Van and Wu \shortcite{DBLP:journals/corr/abs-2311-06737} utilized LMM to identify and correct HS, substituting the text in memes with positive and respectful language.

These studies underscore the critical role of generative models in annotating and developing counter speech strategies. This further signifies the future opportunities of LMMs and LMMs in enhancing approaches and techniques to combat hate speech effectively.
